Bi-Manual Block Assembly via Sim-to-Real Reinforcement Learning

Most successes in robotic manipulation have been restricted to single-arm gripper robots, whose low dexterity limits the range of solvable tasks to pick-and-place, inser-tion, and object rearrangement. More complex tasks such as assembly require dual and multi-arm platforms, but entail a suite of unique challenges such as bi-arm coordination and collision avoidance, robust grasping, and long-horizon planning. In this work we investigate the feasibility of training deep reinforcement learning (RL) policies in simulation and transferring them to the real world (Sim2Real) as a generic methodology for obtaining performant controllers for real-world bi-manual robotic manipulation tasks. As a testbed for bi-manual manipulation, we develop the U-Shape Magnetic BlockAssembly Task, wherein two robots with parallel grippers must connect 3 magnetic blocks to form a U-shape. Without manually-designed controller nor human demonstrations, we demonstrate that with careful Sim2Real considerations, our policies trained with RL in simulation enable two xArm6 robots to solve the U-shape assembly task with a success rate of above90% in simulation, and 50% on real hardware without any additional real-world fine-tuning. Through careful ablations,we highlight how each component of the system is critical for such simple and successful policy learning and transfer,including task specification, learning algorithm, direct joint-space control, behavior constraints, perception and actuation noises, action delays and action interpolation. Our results present a significant step forward for bi-arm capability on real hardware, and we hope our system can inspire future research on deep RL and Sim2Real transfer of bi-manualpolicies, drastically scaling up the capability of real-world robot manipulators.

==> 2000_todos.tex <==

% \sg{We shouldn't have too many Sections as that could make navigation difficult. We should be clear that this is a "system" paper to demonstrate result on a really challening task. i like paper structure like https://taochenshh.github.io/projects/in-hand-reorientation#  https://openreview.net/pdf?id=7uSBJDoP7tY. very simple and clear Section structure}

% \subsection{Task specification}
% put "Connect Task" here?

% observations, actions, reward, ..

% \subsection{Direct Joint-Space Control}

% \subsection{Reinforcement Learning Algorithm}
% PPO, SAC.

% \subsection{Behavior Constraints}

% \subsection{Perception and Actuation Noise}


\yc{Should we specify the dimension of each of the above observations/actions in this section (E)?}\sk{yeah let's addres if we have space (moved to TODO)}
